Adaptive Bridge between Training and Inference for Dialogue

Although exposure bias has been widely studied in some NLP tasks, it faces its unique challenges in dialogue response generation, the representative one-to-various generation scenario. In real human dialogue, there are many appropriate responses for the same context, not only with different expressions, but also with different topics. Therefore, due to the much bigger gap between various ground-truth responses and the generated synthetic response, exposure bias is more challenging in dialogue generation task. What's more, as MLE encourages the model to only learn the common words among different ground-truth responses, but ignores the interesting and specific parts, exposure bias may further lead to the common response generation problem, such as "I don't know" and "HaHa?" In this paper, we propose a novel adaptive switching mechanism, which learns to automatically transit between ground-truth learning and generated learning regarding the word-level matching score, such as the cosine similarity. Experimental results on both Chinese STC dataset and English Reddit dataset, show that our adaptive method achieves a significant improvement in terms of metric-based evaluation and human evaluation, as compared with the state-of-the-art exposure bias approaches. Further analysis on NMT task also shows that our model can achieve a significant improvement.

==> 2_backandtra.tex <==
\section{Background and Traditional Methods}
In this section, we  first introduce the Seq2Seq framework which is popular to many generation tasks, and then we will detail the traditional methods proposed by other researchers. 
\subsection{Seq2Seq Generation Model}
\indent The popular dialogue generation models(DGM) are based on sequence-to-sequence (Seq2Seq)~\cite{sutskever2014sequence} framework, which usually has an encoder to read and encode a context sequence of tokens into a hidden vector, and a decoder used to generate the target response sequence. 
In this work we focus on Transformer-based DGM~\cite{VaswaniSPUJGKP17} as it has excellent performance in text generation. It is worth noting that our method can also be easily applied in other DGM Models, such as LSTM and GRU based DGM models. \\
\indent Assume the training set contained N examples pairs is $\{X^k,Y^k\}_{k=1}^{N}$ ,where $X^k=\{x_{1}^{k},x_{2}^{k},\cdots,x_{S_k}^{k}\}$ is the input sequence and $S_k$ means the length of the context sequence while the target output $Y^k$ is a sequence $\{y_{1}^{k},y_{2}^{k},\cdots,y_{T_k}^{k}\}$ where $T_k$ is the length of the response. All tokens of context and target response sequence are belong to a shared dictionary D which size is V. 
Given a context sequence $\{x_{1}^{k},x_{2}^{k},\cdots,x_{S_k}^{k}\}$, same as the Transformer encoder, it will be encoded to a hidden representation:
\begin{equation}
    H_{e}^{k}=\mathbf{TransEncoder}(x_{1}^{k},x_{2}^{k},\cdots,x_{S_k}^{k})
\end{equation}
\noindent where $H_{e}^{k}$ denotes the representation of context sequence in a hidden space. \\
\indent On the decoder side, response sequence is predicted step by step conditioned on the previous ground-truth tokens $y_{<t}^{k}$ and encoder output $h_{e}^{k}$. At the $t-th$ time step, decoder outputs the probability  $p_{t}^{k}$ over all the tokens in the shared vocabulary:
\begin{equation}
   p_{t}^{k}= \mathbf{TransDecoder}(y_{<t}^{k}, H_{e}^{k})
   \label{equ:transdecodertrain}
\end{equation}
$p_{t}^{k}$ can also be denoted by $p(y_t^k|y_{<t}^k,X^k,\theta)$, where $\theta$ are the parameters of encoder and decoder. The response probability $P(Y^k|X^K,\theta)$ can be calculated by the following formula:
\begin{equation}
    P(Y^k|X^K,\theta) = \prod^{T_k}_{t=1}p(y_t^k|y_{<t}^k,X^k,\theta)
\end{equation}

\noindent where $T_k$ is the target length.\\
\indent Given a set of training examples $D=\{X^k,Y^k\}_{k=1}^{N}$, the stander training objective is to minimize the negative log-likelihood of all the training data:
\begin{equation}
    \theta=\mathop{argmin}\limits_{\theta}\{ L (\theta)\}
\end{equation}

\noindent where
\begin{equation}
    \begin{split}
    L(\theta)&=\sum_{k=1}^{N}-logP(Y^k|X^K,\theta)\\
    &=\sum_{k=1}^{N}\sum_{t=1}^{T_k}{-log}p(y_t^k|y_{<t}^k,X^k,\theta)
    \end{split}
\end{equation}
Different from training time, during inference the decoder predict $t-th$ token's probability ${p_{t}^{k}}^*$ conditioned on the previous predicted tokens ${y_{<t}^{k}}^*$ rather than the ground-truth tokens  $y_{<t}^{k}$. It can be calculated by:
\begin{equation}
   {p_{t}^{k}}^*=\mathbf{TransDecoder}({y_{<t}^{k}}^*, H_{e}^{k})
\end{equation}
where ${p_{t}^{k}}^*=p(y_t^k|{y_{<t}^{k}}^*,X^k,\theta)$, and $\theta$ are the parameters of encoder and decoder after training. 
\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\linewidth]{pic/randomsample.png}
    \caption{The Illustration of the Scheduled Sampling Method }
    \label{fig:randomsample}
\end{figure}
\subsection{Scheduled Sampling(SS)}\label{ch:ScheduledSampling}
The main idea of this method is to randomly sample ground-truth tokens or previous predicted tokens during training time. It is illustrated in Figure~\ref{fig:randomsample}. \\
\indent At the $t-th$ time step, the input token of decoder is sampled from $y_{t-1}^{k}$ with a probability of  $\alpha$ or from the previous predicted token ${y_{t-1}^{k}}^*$ with a probability of $1-\alpha$, then predict the $t-th$ token's probability $p_{t}^{k}$ conditioned on the sampled previous tokens ${y_{<t}^{k}}^{\wedge}=\{{y_{1}^{k}}^{\wedge},{y_{2}^{k}}^{\wedge}\cdots,{y_{t-1}^{k}}^{\wedge} \}$ which may contains both ground truth and predicted tokens.\\
\indent Note that, when $\alpha=1$, the training type is same as before, while when $\alpha=0$, the model is trained as inference. If $\alpha$ is set too high($\approx 1$), the inputs of decoder will almost be ground-truth tokens, and will not be able to cope with the unknown tokens predicted in the reference. On the other hand, if $\alpha$ is set too low($\approx 0$) at the beginning of training, the model will yield tokens randomly, as the model is not well trained, which could lead to slow convergence. Therefore, at training time, the probability $\alpha$ should be high at the beginning and then decreased over the training time steps or epochs increasing. \\
\indent ~\citet{bengio2015scheduled} and ~\citet{zhang-etal-2019-bridging}  used a schedule to decrease $\alpha$ as a function of training time steps or epochs,  it is very similar to decrease the learning rate in most modern SGD approaches. The decay function is defined as follows:
\begin{equation}
    \alpha = \frac{k}{k+exp(n/k)}
\end{equation}
where $k\ge1$ depends on the expected speed of convergence, $n$ is the number of training time steps or the training epochs.


